Back To The Future: On Predicting User Uptime

Correlation in user connectivity patterns is generally considered a problem for system designers, since it results in peaks of demand and also in the scarcity of resources for peer-to-peer applications. The other side of the coin is that these connectivity patterns are often predictable and that, to some extent, they can be dealt with proactively. In this work, we build predictors aiming to determine the probability that any given user will be online at any given time in the future. We evaluate the quality of these predictors on various large traces from instant messaging and file sharing applications. We also illustrate how availability prediction can be applied to enhance the behavior of peer-to-peer applications: we show through simulation how data availability is substantially increased in a distributed hash table simply by adjusting data placement policies according to peer availability prediction and without requiring any additional storage from any peer.

==> application__raker_s_conflicted_copy_2010-05-15_.tex <==

We consider a Chord-like \cite{stoica2001chord} DHT providing a
key-value lookup primitive. Our choice is motivated by the fact that
DHTs are generic infrastructures that can be used both by IM
applications and by file-sharing applications (as in the case of Kad),
mapping straightforwardly to the traces we have at hand. Our
techniques can be anyway implemented on various other classes of
distributed applications. For example, it is straightforward to adapt
the following example to the optimization of data placement in
peer-to-peer file storage systems.

Identifiers and hash values for keys are distributed on a logical
ring, and each information on the DHT is replicated on the $n$ nodes
whose identifiers are the closest successors to the hash of the key in
the ring. For the sake of simplicity, we won't consider security or
maintenance issues due to node turnover (i.e., appearence of new nodes
and old nodes that leave the system forever).

In general, node identifiers in DHTs are chosen via a random or
pseudo-random function. We propose, instead, the application of a
smart policy that maximizes the probability that at least one peer in
each \emph{neighbor set} (i.e., each set of $n$ consecutive nodes in
the ring) will be online at any moment in the future. For example, a
smart replica placement policy would distribute pieces of data between
peers which are frequently online at day and at night in order to
obtain high data availability.

We compute the predicted data availability using the ad-hoc predictor
\mortality{and not counting node mortality} for a neighbor set $N$ and a set of
samples in time $T$ as
$$1 - \frac{\sum_{t\in T}1 - \prod_{n\in
    N}(1-p_{n,t})}{|T|}. \label{eq:data-availability}$$ Since our
    predictors have a weekly period, we limit our analysis to the
    first week after the training period, sampling with a frequency of
    one hour.

Our optimization algorithm works iteratively by repeatedly considering
a couple of random nodes and verifying whether exchanging their
identifiers would enhance, on average, the predicted data availability
for the involved neighbor sets. If so, identifiers get exchanged. The
algorithm proceeds until convergence.

 %% {\color{red}(we stop when the
 %%  availability grows by less than $10^{-20}$ in a number of iterations
 %%  comparable to the network size)}. {\color{red}We also implemented
 %%  simulated annealing \cite{} strategies in order to avoid potential
 %%  problems due to local minima, but in practice we didn't obtain real
 %%  benefits from this compared to our simpler default strategy.}

It is noteworthy that, once the predictors for each node on all
samples in $T$ are computed, the placement algorithm is easily
decentralizable: a random DHT lookup is enough to find a random node,
and the values in Eq. \ref{eq:data-availability} can be obtained based
on local information.

We executed our DHT simulation on the IM and Kad traces with training
period of 1 month, and on Skype with a training period of 1 week. All
results reported result from the averaging of 10 experiment runs. To
set the replication factor $n$, we adopted the smallest value that
satisfies $$1 - (1 - \overline a)^n\geq 0.99,$$ where $\overline a$ is
the average availability observed in the training period. This amounts
to a heuristic policy aiming for a 0.99 ratio of data availability if
user uptime is uncorrelated; applying this formula resulted in a value
of $n=15$ for Kad, $n=11$ for IM and $n=5$ for Skype.

\begin{table}

\begin{centering}

\begin{tabular}{|r||r|r||r|r||r|r|}

\hline

Test & \multicolumn{2}{c||}{{Skype}} & \multicolumn{2}{c||}{{IM}} & \multicolumn{2}{c|}{{Kad}} \\

\cline{2-7}

(days) & Rnd. & Opt. &  Rnd. & Opt. &  Rnd. & Opt. \\

\hline \hline

7 & .9833 & .9929 & .9481 & .9788 & .9823 & .9822 \\

\hline

30 & -- & -- & .9509 & .9813 & .9670 & .9796 \\

\hline

60 & -- & -- & .9494 & .9765 & .9439 & .9606 \\

\hline

120 & -- & -- & .9306 & .9580 & .8918 & .9043 \\

\hline

\end{tabular}

\end{centering}

\caption{DHT simulation: availabilities vs. test period.}
\label{tab:dhtsim}

\end{table}


In Tab. \ref{tab:dhtsim}, we show the results of sampling the
simulated data availability (i.e., the ratio of neighbor sets with at
least one online node) with a granularity of one hour and different
lengths for the test period. Data availability using the optimized id
allocation is consistently better than with a random placement.

We also notice some differences between the datasets: IM has a lower
data availability on the short run, because of the higher correlation
between node availabilities, as apparent from
Figure \ref{fig:uptime}. As the training period grows, the average
availability decreases because of nodes leaving the system forever;
this phenomenon is more noticeable in Kad, due to a higher node
turnover rate in the traces. In a realistic application, such a case
can be handled by periodic maintenance policies.

\begin{figure}
\begin{centering}
\includegraphics[width=\columnwidth]{figures/cumgain}
\par\end{centering}

\caption{\label{fig:dhtsim}DHT simulation: benefits vs. test period.}
\end{figure}

In Fig. \ref{fig:dhtsim} shows the benefits of the optimized
id allocation as compared with the traditional random allocation, in
terms of reduction of unavailability. For example, a 50\%
unavailability reduction means that the probability that a piece of
data is unavailable is halved in the optimized case with respect to
the original random allocation.

As the test period grows, the benefits of the smart allocation policy
decrease, both because some peers leave the system and because other
ones change their behavior. In a real system, periodic data
maintenance and identifier reallocation can be used to maintain good
performances.



==> related.tex <==

Given a \emph{training period} in which the traces of the whole network
are observed, we aim to compute an estimation for the 
\begin{itemize}
\item Our goal: we observe traces for a given training set, and we predict
a probability with which a given user will be online at a given time
in the future.
\item Other works tackle availability prediction, but they handle a completely
different problem, generally focusing on the \emph{session length}.
This is useful in various cases, but doesn't take into account long-term
(daily, weekly, seasonal) connectivity patterns.
\end{itemize}

